On the complexity of cache analysis for different replacement policies

Modern processors use cache memory: a memory access that "hits" the cache returns early, while a "miss" takes more time. Given a memory access in a program, cache analysis consists in deciding whether this access is always a hit, always a miss, or is a hit or a miss depending on execution. Such an analysis is of high importance for bounding the worst-case execution time of safety-critical real-time programs.There exist multiple possible policies for evicting old data from the cache when new data are brought in, and different policies, though apparently similar in goals and performance, may be very different from the analysis point of view. In this paper, we explore these differences from a complexity-theoretical point of view. Specifically, we show that, among the common replacement policies, LRU (Least Recently Used) is the only one whose analysis is NP-complete, whereas the analysis problems for the other policies are PSPACE-complete.

==> PLRU_drawing.tex <==
%% Macro to draw a 4 ways plru cache state.
% First and second parameters are the x and y coordinates of the bottom left corner of the figure.
% Third parameter is the list of ways content, comma separated.
% Fourth parameter is the list of the tree bits from top to bottom, left to right.
% Example : \plrufour{0}{0}{$a$, ,$b$, }{001} draw the following figure at position (0,0)
%
%          0
%        /   \
%       v     \
%      0       1
%     / \     / \
%    v   \   /   v
%  -----------------
%  | a |   | b |   |
%  -----------------
\newcommand{\plrufour}[4]{
	\tikzset{way/.style={draw, rectangle, minimum size=1cm, text height=1.5ex, text depth=.25ex}}
	\tikzset{tree/.style={draw, circle, minimum size=0.8cm, text height=1.5ex, text depth=.25ex}}
	\tikzset{arrow/.style={->, >=stealth}}

	%% Cache content

	% Retrieve ways content from function argument
	\setsepchar{,}
	\readlist\ways{#3}

	\node[way] (w0) at (#1+0,#2+0) {\ways[1]};
	\node[way] (w1) at (#1+1,#2+0) {\ways[2]};
	\node[way] (w2) at (#1+2,#2+0) {\ways[3]};
	\node[way] (w3) at (#1+3,#2+0) {\ways[4]};

	%% Tree nodes
	\node[tree] (p0) at (#1+1.5,#2+2.2) {\StrChar{#4}{1}};

	\node[tree] (p1) at (#1+0.5,#2+1.2) {\StrChar{#4}{2}};
	\node[tree] (p2) at (#1+2.5,#2+1.2) {\StrChar{#4}{3}};

	%% Tree edges

	% Retrieve tree bit values from function argument
	\StrChar{#4}{1}[\bita]
	\StrChar{#4}{2}[\bitb]
	\StrChar{#4}{3}[\bitc]

	% Top level
	\ifthenelse{\bita=0}
	           {\draw[arrow] (p0)--node[above left]{0}(p1);\draw        (p0)--node[above right]{1}(p2);}
	           {\draw        (p0)--node[above left]{1}(p1);\draw[arrow] (p0)--node[above right]{0}(p2);}
	% Second level
	\ifthenelse{\bitb=0}
	           {\draw[arrow] (p1)--node[left]{0}(w0);\draw        (p1)--node[right]{1}(w1);}
	           {\draw        (p1)--node[left]{1}(w0);\draw[arrow] (p1)--node[right]{0}(w1);}
	\ifthenelse{\bitc=0}
	           {\draw[arrow] (p2)--node[left]{0}(w2);\draw        (p2)--node[right]{1}(w3);}
	           {\draw        (p2)--node[left]{1}(w2);\draw[arrow] (p2)--node[right]{0}(w3);}
}



%% Command to draw a 8 ways plru cache state.
% First and second parameters are the x and y position of the bottom left corner of the figure.
% Third parameter is the list of ways content, comma separated.
% Fourth parameter is the list of the tree bits from top to bottom, left to right.
% Example : \plrueight{0}{0}{$a$,$b$, ,$c$, , , ,$d$}{0001111}
\newcommand{\plrueight}[4]{}
%	\tikzset{way/.style={draw, rectangle, minimum size=1cm, text height=1.5ex, text depth=.25ex}}
%	\tikzset{tree/.style={draw, circle, minimum size=0.8cm, text height=1.5ex, text depth=.25ex}}
%	\tikzset{arrow/.style={->, >=stealth}}
%
%	%% Cache content
%
%	% Retrieve ways content from function argument
%	\setsepchar{,}
%	\readlist\ways{#3}
%
%	\node[way] (w0) at (#1+0,#2+0) {\ways[1]};
%	\node[way] (w1) at (#1+1,#2+0) {\ways[2]};
%	\node[way] (w2) at (#1+2,#2+0) {\ways[3]};
%	\node[way] (w3) at (#1+3,#2+0) {\ways[4]};
%	\node[way] (w4) at (#1+4,#2+0) {\ways[5]};
%	\node[way] (w5) at (#1+5,#2+0) {\ways[6]};
%	\node[way] (w6) at (#1+6,#2+0) {\ways[7]};
%	\node[way] (w7) at (#1+7,#2+0) {\ways[8]};
%
%	%% Tree nodes
%	\node[tree] (p0) at (#1+3.5,#2+3.2) {\StrChar{#4}{1}};
%
%	\node[tree] (p1) at (#1+1.5,#2+2.2) {\StrChar{#4}{2}};
%	\node[tree] (p2) at (#1+5.5,#2+2.2) {\StrChar{#4}{3}};
%
%	\node[tree] (p3) at (#1+0.5,#2+1.2) {\StrChar{#4}{4}};
%	\node[tree] (p4) at (#1+2.5,#2+1.2) {\StrChar{#4}{5}};
%	\node[tree] (p5) at (#1+4.5,#2+1.2) {\StrChar{#4}{6}};
%	\node[tree] (p6) at (#1+6.5,#2+1.2) {\StrChar{#4}{7}};
%
%	%% Tree edges
%
%	% Retrieve tree bit values from function argument
%	\StrChar{#4}{1}[\bita]
%	\StrChar{#4}{2}[\bitb]
%	\StrChar{#4}{3}[\bitc]
%	\StrChar{#4}{4}[\bitd]
%	\StrChar{#4}{5}[\bite]
%	\StrChar{#4}{6}[\bitf]
%	\StrChar{#4}{7}[\bitg]
%
%	% Top level
%	\ifthenelse{\bita=0}
%	           {\draw[arrow] (p0)--node[above left]{0}(p1);\draw        (p0)--node[above right]{1}(p2);}
%	           {\draw        (p0)--node[above left]{1}(p1);\draw[arrow] (p0)--node[above right]{0}(p2);}
%	% Second level
%	\ifthenelse{\bitb=0}
%	           {\draw[arrow] (p1)--node[above left]{0}(p3);\draw        (p1)--node[above right]{1}(p4);}
%	           {\draw        (p1)--node[above left]{1}(p3);\draw[arrow] (p1)--node[above right]{0}(p4);}
%	\ifthenelse{\bitc=0}
%	           {\draw[arrow] (p2)--node[above left]{0}(p5);\draw        (p2)--node[above right]{1}(p6);}
%	           {\draw        (p2)--node[above left]{1}(p5);\draw[arrow] (p2)--node[above right]{0}(p6);}
%	% Last level
%	\ifthenelse{\bitd=0}
%	           {\draw[arrow] (p3)--node[left]{0}(w0);\draw        (p3)--node[right]{1}(w1);}
%	           {\draw        (p3)--node[left]{1}(w0);\draw[arrow] (p3)--node[right]{0}(w1);}
%	\ifthenelse{\bite=0}
%	           {\draw[arrow] (p4)--node[left]{0}(w2);\draw        (p4)--node[right]{1}(w3);}
%	           {\draw        (p4)--node[left]{1}(w2);\draw[arrow] (p4)--node[right]{0}(w3);}
%	\ifthenelse{\bitf=0}
%	           {\draw[arrow] (p5)--node[left]{0}(w4);\draw        (p5)--node[right]{1}(w5);}
%	           {\draw        (p5)--node[left]{1}(w4);\draw[arrow] (p5)--node[right]{0}(w5);}
%	\ifthenelse{\bitg=0}
%	           {\draw[arrow] (p6)--node[left]{0}(w6);\draw        (p6)--node[right]{1}(w7);}
%	           {\draw        (p6)--node[left]{1}(w6);\draw[arrow] (p6)--node[right]{0}(w7);}
%}

